An Electrolyte Equation of State Based on openCOSMO-RS: From Aqueous Solutions to Non-Aqueous Systems

Predictive COSMO-RS-based electrolyte models such as COSMO-RS-ES describe electrolyte solutions from quantum-chemical information, but treat the liquid as incompressible and give no access to densities or pressure effects. This work presents openCOSMO-RS-ES-Phi, to our knowledge the first open-source implementation of a predictive electrolyte equation of state based on openCOSMO-RS. It combines the COSMO-RS-based equation of state openCOSMO-RS-Phi with the ion interaction energies and the long-range term of COSMO-RS-ES, which is first refitted on the same simplified short range. With this refit, a dielectric decrement improves the mean ionic activity coefficients (MIAC), whereas a Born term counts the solvation of the ions a second time and is therefore left out. The equation of state then adds only volume, dispersion and temperature parameters of the ions, fitted to aqueous MIAC and densities. openCOSMO-RS-ES-Phi reproduces COSMO-RS-ES in dilute aqueous solutions, improves on it in concentrated ones and also yields solution densities. Extrapolating from aqueous systems, it predicts the MIAC in water + cosolvent mixtures as accurately as the fitted COSMO-RS-ES, as well as the MIAC and bubble points of a benchmark database of water-alcohol-salt systems. Salting-out of organic components is not described as accurately, and salts come out too soluble in organic solvents. Overall, the interaction model developed for COSMO-RS-ES carries over to a large extent to an equation of state, which makes openCOSMO-RS-ES-Phi a sound base model for further development, with ion transfer between solvents as a clear target for fitting to non-aqueous data.

==> latexmkrc <==
# Build SI.aux from SI.tex when main.tex needs it for its \externaldocument
# cross-references (xr-hyper). Overleaf otherwise compiles only main.tex.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    my ($base) = @_;
    # Only from the outer run: the SI run in turn references main.aux and
    # must not start another build. An environment variable marks the inner
    # run, since $root_filename does not reliably name the main file
    # (Overleaf compiles with -jobname=output).
    return 0 if $ENV{XR_EXTERNAL_BUILD};
    return 0 unless -e "$base.tex";
    local $ENV{XR_EXTERNAL_BUILD} = 1;
    # Nonstop and forced, so that an error in SI.tex (a missing figure, say)
    # still leaves an SI.aux with all labels instead of stopping the run.
    system("latexmk -cd -pdf -f -interaction=nonstopmode \"$base\"");
    # Never fail the main build because of the SI: at worst its references
    # show as ??.
    return 0;
}

